Mining CryptoNight-Haven on the Varium C1100 Blockchain Accelerator Card

Cryptocurrency mining is an energy-intensive process that presents a prime candidate for hardware acceleration. This work-in-progress presents the first coprocessor design for the ASIC-resistant CryptoNight-Haven Proof of Work (PoW) algorithm. We construct our hardware accelerator as a Xilinx Run Time (XRT) RTL kernel targeting the Xilinx Varium C1100 Blockchain Accelerator Card. The design employs deeply pipelined computation and High Bandwidth Memory (HBM) for the underlying scratchpad data. We aim to compare our accelerator to existing CPU and GPU miners to show increased throughput and energy efficiency of its hash computations

==> algcode.tex <==
\begin{algorithmic}[1]
\STATE $s \gets Keccak(input)$
\STATE $k\{0-9\} \gets AES\: key\: expansion (s[0-31])$
\COMMENT{Explode}
\STATE $b\{0-7\} \gets s[64-191]$
\FOR{i:=1 \TO 16}
  \FOR{j:=0 \TO 7}
    \FOR{l:=0 \TO 9}
      \STATE $b\{j\}\gets AES\:  round(b\{j\}, k\{l\})$
    \ENDFOR
  \ENDFOR
  \STATE $d\{0-7\} \gets 0$
  \FOR{j:=0 \TO 7}
  \STATE $d\{j\} \gets b\{j\} \oplus b\{j+1\mod 8\}$
  \ENDFOR
  \STATE $b \gets d$
\ENDFOR
\STATE $mem\{0-32767\} \gets 0$
\FOR{i:=0 \TO 32767}
  \FOR{j:=0 \TO 7}
    \FOR{l:=0 \TO 9}
    \STATE $b\{j\}\gets AES\:  round(b\{j\}, k\{l\})$
    \ENDFOR
    \STATE $mem\{8i+j\} \gets b\{j\}$
  \ENDFOR
\ENDFOR
\STATE $a \gets s[0-15] \oplus s[32-47]$ \COMMENT{Shuffle}
\STATE $b \gets s[16-31] \oplus s[48-63]$
\STATE $j \gets a[0-7]$
\FOR{i:=1 \TO 262144}
  \STATE $c \gets mem\{j\}$
  \STATE $c \gets AES\: round (c, a)$
  \STATE $mem\{j\} \gets b \oplus c$
  
  \STATE $d \gets mem\{c[0-7]\}$
  \STATE $a \gets a + (c[0-7] \cdot d[0-7])$
  \STATE $mem\{c[0-7]\} \gets a$
  \STATE $a \gets a \oplus d$
  
  \STATE $n \gets mem\{a[0-7]\}[0-7]$
  \STATE $d \gets mem\{a[0-7]\}[8-11]$
  \STATE $q \gets n / (d | 5)$ \COMMENT{Signed division}
  \STATE $mem\{a[0-7]\} \gets n \oplus q$
  \STATE $j \gets (\NOT d) \oplus q$
  \STATE $b \gets c$
\ENDFOR
\STATE $k\{0-9\} \gets AES\: key\: expansion (s[32-63])$
\COMMENT{Implode}
\STATE $b\{0-7\} \gets s[64-191]$
\FOR{m:=0 \TO 1}
\FOR{i:=0 \TO 32767}
  \FOR{j:=0\TO 7}
    \STATE $b\{j\} \gets b\{j\} \oplus mem\{8i+j\}$
    \FOR{l:=0 \TO 9}
      \STATE $b\{j\}\gets AES\:  round(b\{j\}, k\{l\})$
    \ENDFOR
  \ENDFOR
  \STATE $d\{0-7\} \gets 0$
  \FOR{j:=0 \TO 7}
    \STATE $d\{j\} \gets b\{j\} \oplus b\{j+1\mod 8\}$
  \ENDFOR
  \STATE $b \gets d$
\ENDFOR
\ENDFOR
\FOR{i:= 0 \TO 15}
  \FOR{l:=0 \TO 9}
    \STATE $b\{j\}\gets AES\:  round(b\{j\}, k\{l\})$
  \ENDFOR
  \STATE $d\{0-7\} \gets 0$
  \FOR{j:=0 \TO 7}
    \STATE $d\{j\} \gets b\{j\} \oplus b\{j+1\mod 8\}$
  \ENDFOR
  \STATE $b \gets d$
\ENDFOR
\STATE $s[64-191] \gets b$
\STATE $s\gets Keccak\: permutation(s)$
\STATE $h \gets \{Blake, Skein, JH, Groestl\}(s)$
\RETURN $h(s)$
\end{algorithmic}

